MedDiff: Generating Electronic Health Records using Accelerated Denoising Diffusion Model

Due to patient privacy protection concerns, machine learning research in healthcare has been undeniably slower and limited than in other application domains. High-quality, realistic, synthetic electronic health records (EHRs) can be leveraged to accelerate methodological developments for research purposes while mitigating privacy concerns associated with data sharing. The current state-of-the-art model for synthetic EHR generation is generative adversarial networks, which are notoriously difficult to train and can suffer from mode collapse. Denoising Diffusion Probabilistic Models, a class of generative models inspired by statistical thermodynamics, have recently been shown to generate high-quality synthetic samples in certain domains. It is unknown whether these can generalize to generation of large-scale, high-dimensional EHRs. In this paper, we present a novel generative model based on diffusion models that is the first successful application on electronic health records. Our model proposes a mechanism to perform class-conditional sampling to preserve label information. We also introduce a new sampling strategy to accelerate the inference speed. We empirically show that our model outperforms existing state-of-the-art synthetic EHR generation methods.

==> background.tex <==
\section{Background in Diffusion Models}
% First proposed in \cite{denoise}, diffusion models are a family of latent variable generative models characterized by a forward and a reverse Markov process.
% The forward process gradually adds noise to the original data sample, whereas the reverse process undoes the gradual noising process.
% For the reverse process, the sampling starts with the $T$th noise level, $x_T$, and each timestep produces less-noisy samples, $x_{T-1}, x_{T-2}, ...$ until the final sample $x_0$ is produced.
% In essence, the diffusion model learns the ``denoised" version from $x_{t-1}$ to $x_t$.
%However, the sampling process through this Markov chain is not efficient. 

Ho et al. \cite{ho2020denoising} proposed a specific parameterization of the diffusion model to simplify the training process using a score matching-like loss that minimizes the mean-squared error between the true noise and the predicted noise.
They also note that the sampling process can be interpreted as equivalent to Langevian dynamics, which allows them to relate the proposed denoising diffusion probabilistic models (DDPM) to score-based methods in \cite{score}.
Here, we introduce the forward process, the reverse process, and training of DDPM.

\subsection{Forward Process}
Given a data distribution $\bx_0 \sim q(\bx_0)$, DDPM will gradually add noise to the original data distribution until it loses all the original information and becomes an entirely noisy distribution (as shown by the $x_T$ sample in Figure \ref{fig:medDIFF}). To be more specific, we will convolve $q(\bx_0)$ with an isotropic Gaussian noise $\mathcal{N}(0,\sigsq \bI)$ in T steps to produce a noise corrupted sequence $\sequence$. $\bx_T$ will converge to an isotropic Gaussian distribution as $T\rightarrow \infty$. Under the variance schedule that produces $\sequence$, the distribution is derived as 
\begin{equation}
\begin{aligned}
        q(\bx_{1:T}|\bx_0) &= \prod_{t=1}^{T}q(\bx_{t}|\bx_{t-1}) ,\\
        q(\bx_{t}|\bx_{t-1}) &= \mathcal{N}(\bx_t;\sqrt{1-\beta_t}\bx_{t-1},\beta_{t}\bI)
\end{aligned}
\end{equation}
Using the reparameterization trick introduced in \cite{kingma2013auto}, the following nice property holds according to \cite{ho2020denoising}
\begin{align*}
    q(\bx_{t}|\bx_{0}) = \mathcal{N}(\bx_t;\sqrt{\bal_t}\bx_{0},(1-\bal_{t})\bI),\\
    \quad \bal_t =\prodT \alpha_i ~\text{where}~\alpha_t = 1-\beta_t
\end{align*}
Here $\bal$ controls the scale of noise added at each time step. At the beginning, noise should be small so that it is possible for the model to learn well, e.g., $\beta_1<\beta_2<\dots<\beta_T$ and $\bal_1>\bal_2\dots>\bal_T$.
\subsection{Reverse Process}
Since the forward process defined above is a Markov chain, the true sample can be recreated from Gaussian noise $\bx_T \sim\stdnormal $ by reversing the forward process:
\begin{equation}
\label{eq:reversed-process}
\begin{split}
      p_{\theta}(\bx_{0:T})&:= p(\bx_T)\prodT p_{\theta}(\bx_{t-1}|\bx_{t}),\\ p_{\theta}(\bx_{t-1}|\bx_{t}) &= \mathcal{N}(\bx_{t-1};\bmu_{\theta}(\bx_t,t),\mathbf{\Sigma}_{\theta})(\bx_t,t))
\end{split}
\end{equation}
Ho et al. \cite{ho2020denoising} noticed that using Bayes's rule and conditioning on $\bx_0$, the reverse process has a closed form expression:
\begin{equation}
\label{eq:closed-form}
    \begin{split}
        &q(\bx_{t-1}|\bx_{t},\bx_0) =  \mathcal{N}(\bx_{t-1};\Tilde{\bmu}_{t}(\bx_{t},\bx_0),\Tilde{\beta}_{t}\bI),\\
        \text{where}&\quad \Tilde{\bmu}_{t}(\bx_{t},\bx_0) = \frac{\sqrt{\bal_{t-1}}\beta_{t}}{1-\bal_{t}}\bx_0 + \frac{\sqrt{\alpha_{t}}(1-\bal_{t})}{1-\bal_{t}}\bx_t\\
        \text{and}&\quad \Tilde{\beta}_{t} = \frac{(1-\bal_{t-1})}{1-\bal_{t}}\beta_t
    \end{split}
\end{equation}
\subsection{Training}
Based on the reverse process, the training process is based on optimizing the variational lower bound on the negative log likelihood:
\begin{equation}
\begin{split}
     \Exp[-\loglikelihood] &\le \Exp_{q}\Big[-\log \frac{\Pini}{\Qini}\Big] \\
     &= \Exp_{q}\Big[-\log p(\bx_{T}) - \sum_{t\geq 1}\log \frac{\Pinter}{\Qinter}\Big] =: L
\end{split}
\end{equation}
For variance reduction purpose, the loss can be rewritten as:
\begin{equation}
\label{eq:VLB}
\begin{split}
    \Exp_{q}\Big[\underbrace{D_{KL}(q({\bx_{T}|\bx_{0}})||p(\bx_{T}))}_{L_{T}} &+ \sum_{t\geq 1} \underbrace{D_{KL}(q(\bx_{t-1}|\bx_{t},\bx_0)||\Pinter)}_{L_{t-1}}\\ 
    &- \underbrace{\log p_{\theta}(\bx_0|\bx_1)}_{L_0}   \Big]
\end{split}
\end{equation}
Based on \eqref{eq:reversed-process}, \eqref{eq:closed-form} and \eqref{eq:VLB}, $L_{t-1}$ can be computed as:
\begin{equation}
    L_{t-1} = \Exp_{q}\Big[\frac{1}{2\sigma_{t}^2}\|\Tilde{\bmu}_{t}(\bx_{t},\bx_0) - \bmu_{\theta}(\bx_t,t)\|^2   \Big] + C
\end{equation}
where $C$ is a constant independent of $\theta$. Notice that $\bx_{t}(\bx_0,\bep) = \sqrt{\bal{t}\bx_0} + \sqrt{1-\bal_{t}}\bep$ where $\bep \sim \stdnormal$. Thus if we apply \eqref{eq:closed-form}, the loss can be reformulated as:
\begin{equation}
\resizebox{0.91\hsize}{!}{
$L_{t-1} - C  = \Exp_{\bx_{0},\epsilon}\Big[ \frac{1}{2\sigma_{t}^2}\|\Tilde{\bmu}_{t}\Big(\bx_{t}(\bx_0,\bep), \frac{\beta_t}{\sqrt{1-\bal}}\bep\Big) - \bmu_{\theta}(\bx_t,t)\|^2\Big]$}
\end{equation}
% \begin{equation}
% \begin{split}
%     L_{t-1} - C &= \Exp_{\bx_{0},\epsilon}\Big[ \frac{1}{2\sigma_{t}^2}\|\Tilde{\bmu}_{t}\Big(\bx_{t}(\bx_0,\bep), \frac{1}{\sqrt{\bal}}(\bx_{t}(\bx_0,\bep) - \sqrt{1-\bal_{t}}\bep)\Big) - \bmu_{\theta}(\bx_t,t)\|^2\Big] \\
%     & = \Exp_{\bx_{0},\epsilon}\Big[ \frac{1}{2\sigma_{t}^2}\|\Tilde{\bmu}_{t}\Big(\bx_{t}(\bx_0,\bep), \frac{\beta_t}{\sqrt{1-\bal}}\bep\Big) - \bmu_{\theta}(\bx_t,t)\|^2\Big]
% \end{split}
% \end{equation}
Since $\bx_t$ is accessible during training, DDPM chooses the following parametrization:
\begin{equation}
  \bmu_{\theta}(\bx_t,t) =   \frac{1}{\sqrt{\bal}}\Big(\bx_{t}- \frac{\beta_t}{\sqrt{1-\bal}}\bep_{\theta}(\bx_t,t)\Big)
\end{equation}
Finally, the training is performed based on the following loss function:
\begin{equation}
    \Exp_{\bx_{0},\bep}\Big[ \frac{\beta_t^2}{2\sigma_{t}^2\alpha_{t}(1-\bal)}\|\bep - \bep_{\theta}(\sqrt{\bal}\bx_0 + \sqrt{1-\bal}\bep,t)\|\Big]
\end{equation}
\subsection{Algorithm}
Based on above sections, we can summarize the two key algorithms of DDPM.
Algorithm \ref{suppalg:training-dff} displays the complete training procedure with the simplified objective introduced in \cite{ho2020denoising}.
Algorithm \ref{suppalg:Sampling-dff} illustrates the reverse process sampling procedure, where the goal is to predict the error, $\epsilon$.
\begin{algorithm}
        \SetAlgoLined
        \While{$L> tol$}{
        $\bx_0 \sim q(\bx_0)$\\
        $t_{1},t_{2},\dots,t_{k}\sim Uniform({[T]})$\\
        $\bep \sim \stdnormal$\\
        Perform gradient descent on the mini batch:
        $\sum_{i=1}^{k}\nabla_{\theta}\|\bep - \bep_{\theta}(\sqrt{\bal}\bx_0 + \sqrt{1-\bal}\bep,t)\|^2$
        }
         \caption{DDPM Training}
         \label{suppalg:training-dff}
    \end{algorithm}

\begin{algorithm}
        \SetAlgoLined
      $\bx_{T}\sim\stdnormal$\\
        \For{$t = T,\dots,1$}
        {
        $\bz \sim \stdnormal$ if $t>1$, else $\bz =0$\\
        $\bx_{t-1} = \frac{1}{\sqrt{\bal}}\Big(\bx_{t}- \frac{\beta_t}{\sqrt{1-\bal}}\bep_{\theta}(\bx_t,t)\Big) + \sigma_{t}\bz$
        }
        \Return{$\bx_0$}
         \caption{Sampling}
         \label{suppalg:Sampling-dff}
    \end{algorithm}
    
%\subsection{Comparison with other models}



